Efficient Calling Conventions for Irregular Architectures

We empirically evaluated thousands of different C calling conventions for irregular microcontroller architectures, and found potential for improvement over the calling conventions previously used in the Small Device C Compiler (SDCC). The improvements in code size and speed are substantial enough that SDCC made changes to its default calling convention, breaking ABI compatibility.

==> Makefile <==
MAKEFLAGS += --no-builtin-rules # GNU make has an implciit rule that assumes .p is Pascal source instead of gnuplot script.
LATEXARGS = -file-line-error -halt-on-error
LATEX = xelatex
EPS2PDF = ps2pdf14 -dEPSCrop
PLOTS = size-stm8.pdf score-stm8.pdf size-z80.pdf score-z80.pdf size-r3ka.pdf score-r3ka.pdf
IMAGES = $(PLOTS) stm8-registers.pdf z80-registers.pdf stm8-arguments.pdf z80-arguments.pdf sm83-arguments.pdf r3ka-arguments.pdf

SHELL := /bin/bash

.PHONY: all clean

all: callingconvention.pdf

clean:
	rm -f *.eps $(PLOTS) *.aux *.log *.bbl *.blg *.out size-stm8 size-z80 size-r3ka score-stm8 score-r3ka

callingconvention.pdf: callingconvention.tex callingconvention.bbl $(IMAGES)
	$(LATEX) $(LATEXARGS) $< && xelatex $(LATEXARGS) $<

callingconvention.bbl: callingconvention.tex $(IMAGES) callingconvention.bib
	xelatex $(LATEXARGS) $< && bibtex callingconvention; rm callingconvention.pdf

$(PLOTS): %.pdf: %.eps
	$(EPS2PDF) $<

%.eps: %.p % style.p
	gnuplot $<

%.pdf: %.svg
	inkscape --export-filename $*.pdf $*.svg

size-stm8:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args___ret_a_x_xy_000/size`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args_2a_2x_ret_a_x_xy_callee_000/size`; \
		NOASM_SIZE_NEW=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args_2a_2x_ret_a_x_xy_callee_027/size`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-stm8-trunk/size`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-stm8-breaktheworld/size`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD | bc`; \
		NOASM_RATIO=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD | bc`; \
		RATIO=`echo "scale=6;" 1 - $$SIZE_NEW / $$SIZE_OLD | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;

score-stm8:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args___ret_a_x_xy_000/score`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args_2a_2x_ret_a_x_xy_callee_000/score`; \
		NOASM_SIZE_NEW=`cat ../experiments-stm8/$${BENCHMARKS[$$i]}-sdcc_args_2a_2x_ret_a_x_xy_callee_027/score`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-stm8-trunk/score`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-stm8-breaktheworld/score`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD - 1 | bc`; \
		NOASM_RATIO=`echo "scale=6;" $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD - 1 | bc`; \
		RATIO=`echo "scale=6;" $$SIZE_NEW / $$SIZE_OLD - 1 | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;

size-z80:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args____ret_l_hl_dehl_callee_000/size`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args_al_hlde_hlde_ret_a_de_hlde_callee_000/size`; \
		NOASM_SIZE_NEW=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args_al_hlde_hlde_ret_a_de_hlde_callee_009/size`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-z80-trunk/size`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-z80-breaktheworld/size`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD | bc`; \
		NOASM_RATIO=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD | bc`; \
		RATIO=`echo "scale=6;" 1 - $$SIZE_NEW / $$SIZE_OLD | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;

score-z80:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args____ret_l_hl_dehl_callee_000/score`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args_al_hlde_hlde_ret_a_de_hlde_callee_000/score`; \
		NOASM_SIZE_NEW=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-z80-sdcc_args_al_hlde_hlde_ret_a_de_hlde_callee_009/score`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-z80-trunk/score`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-z80-breaktheworld/score`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD - 1 | bc`; \
		NOASM_RATIO=`echo "scale=6;" $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD - 1 | bc`; \
		RATIO=`echo "scale=6;" $$SIZE_NEW / $$SIZE_OLD - 1 | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;

size-r3ka:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args____ret_l_hl_dehl_callee_000/size`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args_2al_2hl_hlde_ret_a_hl_hlde_callee_000/size`; \
		NOASM_SIZE_NEW=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args_2al_2hl_hlde_ret_a_hl_hlde_callee_009/size`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-r3ka-trunk/size`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-r3ka-breaktheworld/size`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD | bc`; \
		NOASM_RATIO=`echo "scale=6;" 1 - $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD | bc`; \
		RATIO=`echo "scale=6;" 1 - $$SIZE_NEW / $$SIZE_OLD | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;

score-r3ka:
	rm -f $@;\
	BENCHMARKS=(whetstone dhrystone coremark stdcbench); \
	BENCHMARKNAMES=(Whetstone Dhrystone Coremark stdcbench); \
	for i in 0 1 2 3; do \
		NOASM_SIZE_OLD=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args____ret_l_hl_dehl_callee_000/score`; \
		NOASM_SIZE_NEW_NOCALLEE=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args_2al_2hl_hlde_ret_a_hl_hlde_callee_000/score`; \
		NOASM_SIZE_NEW=`cat ../experiments-z80/$${BENCHMARKS[$$i]}-r3ka-sdcc_args_2al_2hl_hlde_ret_a_hl_hlde_callee_009/score`; \
		SIZE_OLD=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-r3ka-trunk/score`; \
		SIZE_NEW=`cat ../experiments-breaktheworld/$${BENCHMARKS[$$i]}-r3ka-breaktheworld/score`; \
		NOASM_RATIO_NOCALLEE=`echo "scale=6;" $$NOASM_SIZE_NEW_NOCALLEE / $$NOASM_SIZE_OLD - 1 | bc`; \
		NOASM_RATIO=`echo "scale=6;" $$NOASM_SIZE_NEW / $$NOASM_SIZE_OLD - 1 | bc`; \
		RATIO=`echo "scale=6;" $$SIZE_NEW / $$SIZE_OLD - 1 | bc`; \
		echo $${BENCHMARKNAMES[$$i]} $$NOASM_RATIO_NOCALLEE $$NOASM_RATIO $$RATIO >> $@; \
	done;


